A duality principle in spin glasses

We prove a duality principle that connects the thermodynamic limits of the free energies of the Hamiltonians and their squared interactions. Under the main assumption that the limiting free energy is concave in the squared temperature parameter, we show that this relation is valid in a large class of disordered systems. In particular, when applied to mean field spin glasses, this duality provides an interpretation of the Parisi formula as an inverted variational principle, establishing a prediction of Guerra.

==> invlat.tex <==


%These are definitions for the preamble of TEX files

%\loadmsbm
%that may be needed for \Bbb (``blackboard bold, Bourbaki'') characters
%\UseAMSsymbols
%
%
%\magnification = \magstep1
\font\tencmmib=cmmib10 \skewchar\tencmmib '60
\newfam\cmmibfam
\textfont\cmmibfam=\tencmmib
\def\Ph{\mathchar'4010}
\def\Ps{\mathchar'4011}
\font\tensmc=cmcsc10
\def\smc{\tensmc}
\def\srm{\sevenrm }
%\font\teneufm=EUFM10
%\font\eighteufm=EUFM10 scaled 800
%\def\Fff#1{\hbox{\teneufm#1}}
%\def\Ffff#1{\hbox{\eighteufm#1}}
\font\tenmsb=msbm10
\font\eightmsb=msbm10 scaled 800
\def\Bbb#1{\hbox{\tenmsb#1}}
\def\Bbbb#1{\hbox{\eightmsb#1}}
%\font\bb=msbm10
%\def{\hbox{\bb N}}
%\def\RR{\hbox{\bb R}}
%\def \NN {{I\kern-.3em N}}
%\def \RR {{I\kern-.3em R}}
\def\bbox{\quad\hbox{\vrule \vbox{\hrule \vskip2pt \hbox{\hskip2pt
\vbox{\hsize=1pt}\hskip2pt} \vskip2pt\hrule}\vrule}}
\def\lessim{\ \lower4pt\hbox{$
\buildrel{\displaystyle <}\over\sim$}\ }
\def\gessim{\ \lower4pt\hbox{$\buildrel{\displaystyle >}
\over\sim$}\ }
\def\n{\noindent}
%\def\P{{\rm P}}
%\def\E{{\rm E}}
%\def\LL{{\cal L}}
\def\n{\noindent}
%\parskip=0.03truein
%\hfuzz=0.2truein
%
%\scriptfont4 = \sevensy
%\scriptscriptfont4 = \fivesy
%\font \gross=cmbx10 scaled \magstep2
%\font \mittel=cmbx10 scaled \magstep0  
%\font \outline=ocrb10f scaled \magstep1 
%\pageno = 1
\def\AA{{\cal A} }
\def\AAA{{\bf A} }
\def\Aap{(A,\AA ,P)}
\def\alf{\alpha}
\def\anorm{\|^.\|}
\def\AP{\it Ann. Probab. \bf}
\def\bbe{\vskip .15pc\hangindent=.5pc\hangafter=1}
\def\BB{{\cal B} }
\def\bxt{\boxtimes}
\def\CC{{\cal C} }
\def\claw{\Rightarrow}
\def\cntr{\centerline}
\def\cosph{\cos\phi}
\def\costh{\cos\theta}
\def\DAN{Dokladi AN Ukr.SSR}
\def\DD{{\cal D} }
\def\dc{{\buildrel {d}\over \longrightarrow}}
\def\defn{\skb\fl Definition\rm. }
\def\dens{\text{dens}}
\def\densC{\dens(\CC)}
\def\Dl{\Delta}
\def\dl{\delta}
\def\dnar{\downarrow}
\def\dpo{d_{P,1}}
\def\dpno{d_{P_n,1}}
\def\dpt{d_{P,2}}
\def\EE{{\Bbb E} }
\def\eee{\ =\ }
\def\eeq{\ \equiv \ }
\def\endp{\vfill\break}
\def\Eng{English transl.:}
\def\eps{\varepsilon}
\def\FF{{\cal F} }
\def\GG{{\cal G} }
\def\gee{\ \ge \ }
\def\goin{\to \infty}
\def\go0{\to 0}
\def\grad{\triangledown}
\def\fl{\smallskip}
%\def\fl{\flushpar} 
\def\HH{{\cal H} }
\def\inv{^{-1}}
\def\JJ{{\cal J} }
\def\KK{{\cal K} }
\def\la{\langle}
\def\li{< \infty}
\def\linF{\ell\upin(\FF)\ }
\def\lm{\lambda}
\def\Lm{\Lambda}
\def\lee{\ \le \ }
\def\leftitem#1{\item{\hbox to\parindent{\enspace#1\hfill}}}
\def\LL{{\cal L} }
\def\Lt{L^2(P)}
\def\Lto{L^2_0(P)}
\def\mc{m^{\CC }(}
\def\mcn{m^{\CC}(n)}
\def\mdsk{\medskip}
\def\mm{\vskip 1mm}
\def\MM{{\cal M} }
\def\nF{\|_{\FF}}
\def\NN{{\cal N} }
\def\normf{\|\cdot\|_{\cal F}}
\def\omg{\omega}
\def\Omg{\Omega}
\def\Omgap{(\Omg,\AA,{\rm Pr})\ }
\def\Omgsp{(\Omg, \Sigma ,{\rm Pr})\ }
\def\Omgspb{(\hat \Omg, \hat \Sigma ,\hat Pr)\ }
\def\Omgspr{(\Omg_{\eps }, \Sigma_{\eps } ,Pr_{\eps })\ }
\def\Omgspp{(\Omg_{\nu }, \Sigma_{\nu } , Pr_{\nu })\ }
\def\OO{{\bf O}}
\def\pard{\partial}
\def\pf{\hfill\break\bf Proof. \rm}
\def\pl{\ + \ }
\def\PP{{\cal P} }
\def\pr{probability}
\def\prm{^{\prime}}
\def\prc{{\buildrel {p}\over \longrightarrow}}
\def\prloc{{\buildrel {p,loc}\over \longrightarrow}}  
\def\prbloc{{\buildrel {{p, bloc}}\over \longrightarrow}}  
\def\qed{\hfill\break\rightline{$\bbox$}}
\def\QQ{{\cal Q}}
\def\ra{\rangle} 
\def\rbar{\overline{\Bbb R}}
\def\refs{\mdsk\cntr {REFERENCES}\mdsk}
\def\RR{{\Bbb R }}
\def\rtar{\Rightarrow}
\def\Ru{(in Russian)\ }
\def\sap{(S,\AA ,P)}
\def\soc{S(\CC )}
\def\setm{\setminus}
\def\sg{\sigma}
\def\sga{$\sigma$-algebra }
\def\sgal{$\sigma$-algebra}
\def\sg2{\sigma^2}
\def\sinph{\sin\phi}
\def\sinth{\sin\theta}
\def\skb{\medskip\fl\bf}
\def\sqt{^{1/2}}
\def\Sp{{\cal SP}(\RR^d)}
\def\SS{{\cal S} }
\def\SSSi{\smallint^{\infty}}
\def\SSOI{\smallint^1_0}
\def\SSS{\smallint}
\def\SSSW{\smallint^{\infty}_{-\infty}}
\def\tens{\otimes}
\def\TVMS{Teoria verojatnostej i matemati\v ceskaia statistika }
\def\TPA{\it Theor. Probability Appl. \bf}
\def\TPMS{Probability Theory and Mathematical Statistics, American
Mathematical Society} 
\def\tpr{\text{Pr}}
\def\TT{{\cal T} }
\def\subin{\_{\infty}}
\def\sumi{\sum^{\infty}}
\def\UMZ{Ukrainskij matemati\v ceskij \v zurnal}
\def\upar{\uparrow}
\def\upin{^{\infty}}
\def\VV{{\cal V}} 
\def\vc{Vapnik-\v Cervonenkis\ }
\def\wc{{\buildrel {w}\over \longrightarrow}}
\def\wloc{{\buildrel {w,loc}\over \longrightarrow}}  
\def\wbloc{{\buildrel {w, bloc }\over \longrightarrow}} 
\def\WW{{\cal W} } 
\def\XX{{\bf X} }
\def\xa{(\XX,\AA )\ }
\def\xap{(\XX,\AA,P)\ }
\def\xy{\{x,y\}}
\def\ZW{\it Z. Wahrscheinlichkeitsth. verw. Geb. \bf}
\def\ZZ{{\cal Z} }
\def\__{_{\infty}}
%\medskipamount=6pt plus 2pt minus 2pt










